Computing Distances between Reach Flowpipes

We investigate quantifying the difference between two hybrid dynamical systems under noise and initial-state uncertainty. While the set of traces for these systems is infinite, it is possible to symbolically approximate trace sets using \emph{reachpipes} that compute upper and lower bounds on the evolution of the reachable sets with time. We estimate distances between corresponding sets of trajectories of two systems in terms of distances between the reachpipes. In case of two individual traces, the Skorokhod distance has been proposed as a robust and efficient notion of distance which captures both value and timing distortions. In this paper, we extend the computation of the Skorokhod distance to reachpipes, and provide algorithms to compute upper and lower bounds on the distance between two sets of traces. Our algorithms use new geometric insights that are used to compute the worst-case and best-case distances between two polyhedral sets evolving with time.

==> frechet-pipe.tex <==
\section{Fr{\'e}chet  Distances between Polytope-Reachpipes}
\label{section:FrechetPipe}

In Subsection~\ref{subsection:ReachpipeConstruction}
we  discuss appropriate representations of reachpipes, and then
in Subsections~\ref{subsection:PipeToPoly-One} and~\ref{subsection:PipeToPoly-Two},
we discuss
distances when reachpipes are viewed as set valued traces.

\RM{At some point you move from arbitrary time points $t_0, \ldots, t_{m-1}$ 
to time points that are the integers $0,\ldots,m-1$.
Needs fixing.}

\subsection{Constructing Reachpipes}
\label{subsection:ReachpipeConstruction}

Our  Skorokhod distance computation procedure will operates on reachpipes,
it is thus necessary to choose an appropriate model of reachpipes so that the 
distance computation procedure remains tractable.
Recall that a reachpipe $R$ is a mapping  from
finite closed interval $[T_i,T_e]$ to subsets if $\reals^d$.
For a reachpipe $R$ over the time interval $[0,T]$, the points in the set 
$R(t)$ denote the possible trace values that can occur.
A reachpipe  thus consists of   time-varying subsets of $\reals^d$.
Also recall that  Algorithm~\ref{algo:DistancePipe} requires that 
given reachpipe samples $R(t_0), \dots, R(t_m)$, we be able to
``complete'' the reachpipes for intermediate time values.
We do this completion by generalizing linear interpolation using
scaling and Minkowski sums.


\smallskip\noindent\textbf{Reachpipe Completion.}
Suppose there is a trace $\pi$ such that we observe $f(t_k) = \bp$ and
$f(t_{k+1}) = \bp'$ via sampling.
It is customary to complete the trace $f$ using standard interpolation schemes
eg., linear interpolation.
In our framework,  the reachpipe set  sample $R(t_k)$ represents the fact that
every  $\bp\in R(t_k)$ occurs in some trace in the original tracepipe.
Since every point in $R(t_k)$ and $R(t_{k+1})$ occurs in some sampling, we
obtain an over-approximated completion of $R$ in between $t_k, t_{k+1}$ as follows
for $t_k \leq t \leq t_{k+1}$:
\[
\mspace{-10mu}
\ceil{R(t)} = \left\{ 
\bp + \frac{t-t_k}{t_{k+1}-t_k}
\vdot (\bq- \bp)\  \Big\arrowvert\ 
\bp\in  R(t_k) \text{ and } \bq\in  R(t_{k+1})  \right\}.
\]
For a set $A\subseteq \reals^d$,
given $\lambda \in \reals$,  let $\lambda\cdot A$ denote
$\set{\lambda\cdot \bp \mid \bp\in A}$.
The Minkowski sum of two sets $A, B$ is defined as
$A+B = \set{\bp+\bq \mid \bp \in A \text{ and } \bq \in B}$.
We also denote $-1 \cdot A$ by $-A$.
Under this notation, we have
\begin{equation}
\label{equation:CompletionOver}
\ceil{R(t)} = R(t_k) + \frac{t-t_k}{t_{k+1}-t_k}\cdot\left(R(t_{k+1})  - R(t_{k})\right).
\end{equation}
We explain why the above is an over-approximation even if we assume linear 
interpolation completions of observed trace samples.
Recall that 
\[R(t)  = \set{\bp \mid \text{ there exists some trace } f \text{ such that }
f(t) = \bp}.\]
Under linear interpolation completion of traces, this set is
\begin{equation}
\label{equation:CompletionExact}
R(t)  = \left\{\bp + \frac{t-t_k}{t_{k+1}-t_k}
\vdot (\bq- \bp)\  \bigg\arrowvert
\begin{array}{l}
\text{ there exists a trace } f\\
 \text{ such that }
f(t_k) = \bp \text{ and }\\
 \ f(t_{k+1}) = \bq
\end{array}
\mspace{-15mu}
\right\}
\end{equation}


In general $R(t) $ as defined in
Equation~\ref{equation:CompletionExact}
 can be a strict subset of $\ceil{R(t)}$ as defined in 
Equation~\ref{equation:CompletionOver}.
\begin{figure}[h]
\begin{minipage}[t]{0.2\textwidth}
\picfile{completion-1.eepic}
\end{minipage}
%$\qquad$
\begin{minipage}[t]{0.2\textwidth}
\picfile{completion-2.eepic}
\end{minipage}
\caption{Reachpipe Completion (i) $R(t) $; (ii) $\ceil{R(t)}$}
\label{figure:ReachpipeCompletion}
\end{figure}
For an example, see Figure~\ref{figure:ReachpipeCompletion}, where
$R(t_k) \subseteq \reals$ and $ R(t_{k+1})\subseteq \reals$ are the 
disjoint black line segments
at the ends, and the shaded portions are the completions for $t\in (t_k, t_{k+1})$.


\smallskip\noindent\textbf{Reachpipe Sample Sets.}
We now look at choosing appropriate forms of 
reachpipe sample sets $R(t_k)$.
In hybrid systems literature the common forms of reach sets are
(i)~ellipsoids~\cite{KurzhanskiV06}, 
(ii)~support functions~\cite{GuernicG10},
(iii)~zonotopes~\cite{Girard05,GirardG08},
(iv)~polyhedra and 
polytopes~\cite{FrehseGDCRLRGDM11,HanK06,ChutinanK03,SankaranarayananDI08,SankaranarayananDI08,ColonS11},
(v)~polynomial approximations~\cite{PrabhakarV11, ChenAS12}.

In this work we use  polytopes as reachpipe sample sets (in this paper, polytopes 
are taken to mean convex polytopes.
A \emph{polyhedron} is specified as:
$A\cdot \bx \leq  \bb$, where
$A$ is a $n \times d$ real-valued matrix, 
$\bx = [x_1, \dots, x_d]^{\transpose}$ is a column vector of $d$ variables,
$\bb =  [b_1, \dots, b_d]^{\transpose}$ is a column vector with $b_k\in \reals$ for 
every $k$, and ``$\cdot$" denotes the standard matrix product.
The polyhedron $A\cdot \bx \leq  \bb$ consists of all points
$(p_1, \dots, p_d) \in \reals^d$ such that for all $1\leq i \leq n$, we have 
$\sum_{k=1}^d A_{i,k}\cdot p_k \leq b_k$.
A polyhedron is thus the intersection of $n$ halfspaces, namely, the halfspaces
$\sum_{k=1}^d A_{i,k}\cdot x_k \leq b_k$ for $1\leq i \leq n$.
We use $\ba_i\cdot \bx \leq b_i$ as a shorthand to denote the $i$-th halfspace, where
$\ba_i$ is the $i$-th row vector of $A$.
A \emph{polytope} is a bounded polyhedron.
Polytopes can also be specified as convex hulls of  a finite set of 
points~\cite{ZieglerBook}.
Unfortunately, polynomial time algorithms are not known to obtain  one representation
from the other~\cite{WelzlABS97}.
We use the halfspace representation as  it has been shown to have been 
 amenable to computing
over-approximations of reach sets of hybrid systems using the template polyhedra 
approach~\cite{HanK06,ChutinanK03,SankaranarayananDI08,SankaranarayananDI08,ColonS11}.
The reachsets at  sampled  timepoints is over-approximated by polytopes
by varying the constants in $\bb$, 
the matrix $A$ stays unchanged.
Zonotopes are special forms of polytopes, the algorithms developed in this work are also
applicable for these special polytopes.

We note the property that if  $R(t_k)$ and $R(t_{k+1})$ are polytopes (resp. zonotopes)
in Equation~\ref{equation:CompletionOver}, 
the completions $\ceil{R(t)}$ for every $t$ are also  polytopes (resp. zonotopes).
This follows from the facts that for $P_1$ and $P_2$ polytopes (resp. zonotopes),
(i)~$\lambda\cdot P_1$ and  $\lambda\cdot P_2$ are  polytopes (resp. zonotopes)
for $\lambda$ a constant; and
(ii)~the Minkowski sum $P_1 + P_2$ is also a polytope (resp. zonotope)~\cite{ZieglerBook}.




\smallskip\noindent\textbf{Polygonal Polytope-Reachpipe (\ppr).}
A \emph{polygonal polytope-reachpipe} (\ppr) is a reachpipe specified
by reachpipe time-samples $R(0),\dots R(m)$, such that for $k\in \set{0,1,\dots m-1}$ 
(a)~each $R(k)$ is a polytope of $\reals^{d+1}$; and
(b)~$R(t)$ for $k < t < k+1$  is taken to be
 the linear interpolation as specified in Equation~\ref{equation:CompletionOver}.
Note that we take the reachpipe samples to occur at integer parameter values,
this is WLOG as the actual time value has been added as an extra dimension as
discussed in Subsection~\ref{subsection:MovingFrechet}.
Next,  we study the variation distance between  \ppr{s}
with respect to the \frechet trace metric.

%\newpage
\subsection{From Pipe Variation Distances to Polytope-Trace Distances}
\label{subsection:PipeToPoly-One}

Let $R_1, R_2$ be \pprs from $[0, m_1]$ and $[0, m_2]$ to
polytopes over  $\reals^{d+1}$.
Our objective is to 
bound the tracepipe variation distance with respect to the \frechet trace  metric.
From Proposition~\ref{proposition:OverUnder}, we
need to compute 
(a)~$\dvarfre\left(F^{R_1}, F^{R_2}\right)$
(recall from Section~\ref{subsection:Basic} that given a reachpipe $R$, the 
corresponding tracepipe is denoted $F^R$);
and 
(b)~$\dist_{\min}\left(F^{R_1}, F^{R_2}\right)$.

In this subsection, we deal with the first case, ie., $\dvarfre\left(F^{R_1}, F^{R_2}\right)$.
Recall that this value is defined as:
\begin{equation}
\label{equation:TracepipeRef}
\dvarfre\left(F^{R_1}, F^{R_2}\right) =
 \sup_{f_1\in F^{R_1}, f_2\in F^{R_2}} \dist_{\fre}(f_1, f_2)
\end{equation}

We define a new variation distance on reachpipes as follows.
\begin{definition}
\label{definition:ReachpipeFre}
Let $R_1, R_2$ be \pprs from $[0, m_1]$ and $[0, m_2]$ to
polytopes over $\reals^{d+1}$, and let $L$ be a given norm on
$\reals^{d+1}$.
The reachpipe variation distance
$\dvarfre^{\dagger}\left(R_1, R_2\right) $ is defined as:
\begin{equation}
\label{equation:ReachpipeFre}
%\dvarfre\left(R_1, R_2\right) =
 \inf_{\substack{
\alpha_1: [0,1] \rightarrow [0, m_1] \\
\alpha_2: [0,1] \rightarrow [0, m_2] }}
\max_{0\leq \theta \leq 1} \quad
\max_{\bp_1\in R_1\left(\alpha_1(\!\theta\!)\right),\ 
\bp_2\in R_2\left(\alpha_2(\!\theta\!)\right)}
\norm{\bp_1-\bp_2}_{L}
\end{equation}
where $\alpha_1, \alpha_2$ range over  continuous and strictly increasing bijective functions
onto  $[0, m_1]$ and $[0, m_2]$ respectively.\qed
\end{definition}
Note that $\dvarfre^{\dagger}$ is defined over \emph{reachpipes} $R$,
as compared to $\dvarfre$ which is defined over tracepipes
$F$ or $F^R$.
Also note that for any reparametrizations $\alpha_1, \alpha_2$, the sets 
$R_1\left(\alpha_1(\theta)\right)$ and $R_2\left(\alpha_2(\theta)\right)$
are closed and bounded.
Thus, $\max_{\bp_1\in R_1\left(\alpha_1(\!\theta\!)\right),\ 
\bp_2\in R_2\left(\alpha_2(\!\theta\!)\right)}
\norm{\bp_1-\bp_2}_{L}$ is well defined.
The function $\dvarfre^{\dagger}$, like the function $\dvarfre$, is not a metric
(notably, we can have $\dvarfre^{\dagger}(R,R) > 0$).


Informally, we go along both the \pprs $R_1, R_2$ according to our chosen
 reparametrizations $\alpha_1, \alpha_2$, and compare the \emph{polytopes}
$R_1\left(\alpha_1(\theta)\right)$ and $R_2\left(\alpha_2(\theta)\right)$
for each value of $0\leq \theta\leq 1$. 
If we view a \ppr $R$ as a mapping from $[0, m]$ to the set of
polytopes of $\reals^{d+1}$, then 
Definition~\ref{definition:ReachpipeFre} seems similar to the 
definition of the \frechet distance over 
traces~\ref{def:frechet}, where we use the following function to compare
polytopes $P_1, P_2$:
\begin{equation}
\label{equation:PhiMax}
  \Phi_{\max}(P_1, P_2) = \max_{\bp_1\in P_1, \bp_2\in P_2}\norm{\bp_1- \bp_2}_L
\end{equation}
Using $\Phi_{\max}$, 
Equation~\ref{equation:ReachpipeFre} can be written as:
\begin{equation}
\dvarfre^{\dagger}\!\left(R_1, R_2\right) =
%\dvarfre\left(R_1, R_2\right) =
 \inf_{\substack{
\alpha_1: [0,1] \rightarrow [0, m_1] \\
\alpha_2: [0,1] \rightarrow [0, m_2] }}
\max_{0\leq \theta \leq 1} \Phi_{\max}\Big(
R_1\!\left(\alpha_1(\!\theta\!)\right),\,
R_2\!\left(\alpha_2(\!\theta\!)\right)
\Big)
\end{equation}

The following theorem shows that $\dvarfre^{\dagger}\!\left(R_1, R_2\right)$
%is actually equal to the tracepipe distance
over-approximates the tracepipe distance
$\dvarfre\left(F^{R_1}, F^{R_2}\right)$.
%
\begin{theorem}
\label{theorem:ReachpipeFreVar}
Let $R_1, R_2$ be \pprs from $[0, m_1]$ and $[0, m_2]$ to
polytopes over $\reals^{d+1}$, and let $L$ be a given norm on
$\reals^{d+1}$.
We have
\[
\dvarfre^{\dagger}\!\left(R_1, R_2\right) \ \geq \ 
\dvarfre\left(F^{R_1}, F^{R_2}\right)
\]
where the tracepipe distance $\dvarfre\left(F^{R_1}, F^{R_2}\right)$ is
as defined in
\ref{equation:TracepipeRef},
and the reachpipe distance $\dvarfre^{\dagger}\!\left(R_1, R_2\right)$
  is as defined in Definition~\ref{definition:ReachpipeFre}.
\end{theorem}
\begin{proof}
%\begin{enumerate}
%\item 
%$\dvarfre^{\dagger}\!\left(R_1, R_2\right) \geq \dvarfre\left(F^{R_1}, F^{R_2}\right)$.\\
Consider any $f_1\in  F^{R_1}$, and any  $f_2\in  F^{R_2}$.
We have 
\[
\mspace{-20mu}
\dist_{\fre}(f_1, f_2) =  \inf_{\substack{
\alpha_1: [0,1] \rightarrow [0, m_1] \\
\alpha_2: [0,1] \rightarrow [0, m_2] }}\ 
\max_{0\leq \theta \leq 1} \norm {f_1\left(\alpha_1(\theta)\right) - f_2\left(\alpha_2(\theta)\right)}
\]
Observe that
$f_j\left(\alpha_j(\theta)\right) \in R_j\left(\alpha_j(\theta)\right)$ for $j\in\set{1,2}$.
Thus, for every $\alpha_1, \alpha_2, \theta$, 
\[
\norm {f_1\left(\alpha_1(\theta)\right) - f_2\left(\alpha_2(\theta)\right)}
\leq 
 \Phi_{\max}\left(
R_1\left(\alpha_1(\theta)\right), \, R_2\left(\alpha_2(\theta)\right)
\right)
\]
Thus, we have
\[
\dist_{\fre}(f_1, f_2) \leq  \inf_{\substack{
\alpha_1: [0,1] \rightarrow [0, m_1] \\
\alpha_2: [0,1] \rightarrow [0, m_2] }}\ 
\max_{0\leq \theta \leq 1}
\Phi_{\max}\Big(
R_1\!\left(\alpha_1(\!\theta\!)\right),\,
R_2\!\left(\alpha_2(\!\theta\!)\right)
\Big)
\]
That is, for every $f_1\in  F^{R_1}$, and  $f_2\in  F^{R_2}$, we have
$\dist_{\fre}(f_1, f_2)  \leq \dvarfre^{\dagger}\!\left(R_1, R_2\right)$.
This implies that 
$\sup_{f_1\in F^{R_1}, f_2\in F^{R_2}} \dist_{\fre}(f_1, f_2)
\leq \dvarfre^{\dagger}\!\left(R_1, R_2\right)$.
%
\begin{comment}
\item 
$\dvarfre^{\dagger}\!\left(R_1, R_2\right) \leq \dvarfre\left(F^{R_1}, F^{R_2}\right)$.\\
Informally, we need to construct curves $f_1^*, f_2^*$ such that
for all $\rho_1\in [0, m_1]$ and for all $\rho_2\in [0, m_2]$, we have that
$\Phi_{\max}\left( R_1(\rho_1), R_2(\rho_2)\right) \leq \norm{f_1^*(\rho_1), f_2^*(\rho_2)}$.
If we can obtain such curves, then we would have that
\[
\begin{array}{c}
 \inf_{\substack{
\alpha_1: [0,1] \rightarrow [0, m_1] \\
\alpha_2: [0,1] \rightarrow [0, m_2] }}
\max_{0\leq \theta \leq 1} \Phi_{\max}\Big(
R_1\!\left(\alpha_1(\!\theta\!)\right),\,
R_2\!\left(\alpha_2(\!\theta\!)\right)
\Big)\\ 
\leq \\
 \inf_{\substack{
\alpha_1: [0,1] \rightarrow [0, m_1] \\
\alpha_2: [0,1] \rightarrow [0, m_2] }}
\max_{0\leq \theta \leq 1}
\norm{f_1^* \!\left(\alpha_1(\!\theta\!)\right) - 
f_2^*\!\left(\alpha_2(\!\theta\!)\right)}
\end{array}
\]
from the fact that for every $\alpha_1, \alpha_2, \theta$,
\[
\Phi_{\max}\Big(
R_1\!\left(\alpha_1(\!\theta\!)\right),\,
R_2\!\left(\alpha_2(\!\theta\!)\right)
\Big)\  \leq\  \norm{f_1^*\!\left(\alpha_1(\!\theta\!)\right) - 
f_2^*\!\left(\alpha_2(\!\theta\!)\right)}
\]
\end{enumerate}
\end{comment}
%
% \mynote{VP: I think the other direction is also true, 
% ie., we should have equality in the theorem,
%  but I have not been able to prove it yet.}
\qedhere
\end{proof}



\subsection{The Minimum Polytope-Trace Distance}
\label{subsection:PipeToPoly-Two}

In Section~\ref{subsection:PipeToPoly-One}, we looked at the value
$\dvarfre\left(F^{R_1}, F^{R_2}\right)$.
In this section, we explore the proximity
distance $\dist_{\min}\left(F^{R_1}, F^{R_2}\right)$
for $R_1, R_2$  two \pprs from $[0, m_1]$ and $[0, m_2]$ to
polytopes over  $\reals^{d+1}$ (as in Section~\ref{subsection:PipeToPoly-One}).
This distance is equal to:
\begin{equation}
\label{equation:TracepipeMinRef}
\dminfre\left(F^{R_1}, F^{R_2}\right) =
 \inf_{f_1\in F^{R_1}, f_2\in F^{R_2}} \dist_{\fre}(f_1, f_2)
\end{equation}
Analogous to the $\dvarfre$ function of
Definition~\ref{definition:ReachpipeFre},
we define a proximity distance  $\dminfre$ over reachpipes.
We use the following function to compare polytopes
(given a norm $L$ over $\reals^{d+1}$):
\begin{equation}
\label{equation:PhiMin}
  \Phi_{\min}(P_1, P_2) = \min_{\bp_1\in P_1,\, \bp_2\in P_2}\norm{\bp_1- \bp_2}_L
\end{equation}
Using this function, we define $\dminfre$ as follows.
%
\begin{definition}
\label{definition:ReachpipeMinFre}
Let $R_1, R_2$ be \pprs from $[0, m_1]$ and $[0, m_2]$ to
polytopes over $\reals^{d+1}$, and let $\Phi_{\min}$ be the
polytope comparison function as described previously.
The reachpipe proximity distance
$\dminfre^{\dagger}\left(R_1, R_2\right) $ is defined as:
\begin{equation}
\dminfre^{\dagger}\!\left(R_1, R_2\right) =
%\dvarfre\left(R_1, R_2\right) =
 \inf_{\substack{
\alpha_1: [0,1] \rightarrow [0, m_1] \\
\alpha_2: [0,1] \rightarrow [0, m_2] }}
\max_{0\leq \theta \leq 1} \Phi_{\min}\Big(
R_1\!\left(\alpha_1(\!\theta\!)\right),\,
R_2\!\left(\alpha_2(\!\theta\!)\right)
\Big)
\end{equation}
where $\alpha_1, \alpha_2$ range over  continuous and strictly increasing bijective functions
onto  $[0, m_1]$ and $[0, m_2]$ respectively.\qed
\end{definition}
The following theorem shows that $\dminfre^{\dagger}\!\left(R_1, R_2\right)$
is equal to the  tracepipe distance
$\dminfre\left(F^{R_1}, F^{R_2}\right)$.
The proof of the theorem can be found in the Appendix.
%
\begin{theorem}
\label{theorem:ReachpipeFreMin}
Let $R_1, R_2$ be \pprs from $[0, m_1]$ and $[0, m_2]$ to
polytopes over $\reals^{d+1}$, and let $L$ be a given norm on
$\reals^{d+1}$.
We have
\[
\dminfre^{\dagger}\!\left(R_1, R_2\right) \ = \ 
\dminfre\left(F^{R_1}, F^{R_2}\right)
\]
where the tracepipe distance $\dminfre\left(F^{R_1}, F^{R_2}\right)$ is
as defined in
\ref{equation:TracepipeMinRef},
and the reachpipe distance $\dminfre^{\dagger}\!\left(R_1, R_2\right)$
  is as defined in Definition~\ref{definition:ReachpipeMinFre}.
\qed
\end{theorem}
\begin{comment}
\begin{proof}
We prove inequalities in both directions.

\medskip\noindent
(1)~$\dminfre\left(F^{R_1}, F^{R_2}\right) \geq \dminfre^{\dagger}\!\left(R_1, R_2\right) $.\\
Consider any $f_1\in  F^{R_1}$, and any  $f_2\in  F^{R_2}$.
We have 
\[
\mspace{-20mu}
\dist_{\fre}(f_1, f_2) =  \inf_{\substack{
\alpha_1: [0,1] \rightarrow [0, m_1] \\
\alpha_2: [0,1] \rightarrow [0, m_2] }}\ 
\max_{0\leq \theta \leq 1} \norm {f_1\left(\alpha_1(\theta)\right) - f_2\left(\alpha_2(\theta)\right)}
\]
As in the proof of Theorem~\ref{theorem:ReachpipeFreVar},
we have that 
for every $\alpha_1, \alpha_2, \theta$, 
\[
\norm {f_1\left(\alpha_1(\theta)\right) - f_2\left(\alpha_2(\theta)\right)}
\geq 
 \Phi_{\min}\left(
R_1\left(\alpha_1(\theta)\right), \, R_2\left(\alpha_2(\theta)\right)
\right)
\]
Thus, for every $f_1\in  F^{R_1}$, and  $f_2\in  F^{R_2}$, we have
\[
\dist_{\fre}(f_1, f_2) \geq  \inf_{\substack{
\alpha_1: [0,1] \rightarrow [0, m_1] \\
\alpha_2: [0,1] \rightarrow [0, m_2] }}\ 
\max_{0\leq \theta \leq 1}
\Phi_{\min}\Big(
R_1\!\left(\alpha_1(\!\theta\!)\right),\,
R_2\!\left(\alpha_2(\!\theta\!)\right)
\Big)
\]
i.e., $\dist_{\fre}(f_1, f_2)  \geq \dminfre^{\dagger}\!\left(R_1, R_2\right)$.
This implies that 
$\inf_{f_1\in F^{R_1}, f_2\in F^{R_2}} \dist_{\fre}(f_1, f_2)
\geq \dminfre^{\dagger}\!\left(R_1, R_2\right)$.
This completes the proof of the first direction.

\medskip\noindent
(2)~$\dminfre\left(F^{R_1}, F^{R_2}\right) \leq \dminfre^{\dagger}\!\left(R_1, R_2\right) $.\\
Recall that $\dminfre\left(F^{R_1}, F^{R_2}\right)  =$
\[
 \inf_{f_1\in F^{R_1}, f_2\in F^{R_2}}
 \inf_{\substack{
\alpha_1: [0,1] \rightarrow [0, m_1] \\
\alpha_2: [0,1] \rightarrow [0, m_2] }}\ 
\max_{0\leq \theta \leq 1} \norm {f_1\left(\alpha_1(\theta)\right) - f_2\left(\alpha_2(\theta)\right)}.
\]
This equals (switching the $\inf$ order):
\[
 \inf_{\substack{
\alpha_1: [0,1] \rightarrow [0, m_1] \\
\alpha_2: [0,1] \rightarrow [0, m_2] }}\ 
 \inf_{f_1\in F^{R_1}, f_2\in F^{R_2}}\ 
\max_{0\leq \theta \leq 1} \norm {f_1\left(\alpha_1(\theta)\right) - f_2\left(\alpha_2(\theta)\right)}.
\]
We need to show that the above expression is $\leq$ than:
\[
\inf_{\substack{
\alpha_1: [0,1] \rightarrow [0, m_1] \\
\alpha_2: [0,1] \rightarrow [0, m_2] }}\ 
\max_{0\leq \theta \leq 1}\  \Phi_{\min}\Big(
R_1\!\left(\alpha_1(\!\theta\!)\right),\,
R_2\!\left(\alpha_2(\!\theta\!)\right)
\Big)
\]
To show this direction of the inequality, it suffices to show that
for every pair of valid reparametrizations $\alpha_1, \alpha_2$, we have:
\begin{multline}
\label{equation:MinInqTheoremProof}
%\begin{array}{c}
\inf_{f_1\in F^{R_1}, f_2\in F^{R_2}}\ 
\max_{0\leq \theta \leq 1} \norm {f_1\left(\alpha_1(\theta)\right) - f_2\left(\alpha_2(\theta)\right)}\\[-1.5mm]
\leq\\[-1mm]
\max_{0\leq \theta \leq 1}\  \Phi_{\min}\Big(
R_1\!\left(\alpha_1(\!\theta\!)\right),\,
R_2\!\left(\alpha_2(\!\theta\!)\right)
\Big)
\end{multline}
%
The formal proof of the above inequality is technical.

\mynote{VP: Now I handwave.
Is there a simpler proof?}

We sketch the main ideas.
Fix $\alpha_1, \alpha_2$ reparametrizations.
Define the function $\minpairs$  from $ [0,1] $ to
subsets of $\reals^{d+1} \times \reals^{d+1}$ as
 $\minpairs(\theta) =$
\[
\left\{
\tuple{\bp_1, \bp_2} \ \left\arrowvert\ 
\begin{array}{l}
\bp_1\in R_1\!\left(\alpha_1(\theta)\right),
\text{ and } 
\bp_2\in R_2\!\left(\alpha_2(\theta)\right),\\
\text{ and }
\norm{\bp_1-\bp_2} \leq \Phi_{\min}
\Big(
R_1\!\left(\alpha_1(\!\theta\!)\right),\,
R_2\!\left(\alpha_2(\!\theta\!)\right)
\Big)
\end{array}
\right.\mspace{-10mu}\right\}
\]  
That is, $\minpairs(\theta)$ contains point pairs
$\tuple{\bp_1, \bp_2}$ with $\bp_1\in R_1\!\left(\alpha_1(\theta)\right)$,
and 
$\bp_2\in R_2\!\left(\alpha_2(\theta)\right)$ such that
$\bp_1, \bp_2$ are the closest points in the corresponding polytopes
$ R_1\!\left(\alpha_1(\theta)\right)$ and 
$R_2\!\left(\alpha_2(\theta)\right)$
(there may be several such pairs for the two polytopes).
It can be shown that for each $\theta$, we can pick a single point tuple
from $\minpairs(\theta) $, namely
$\tuple{\bp_1^{\theta}, \bp_2^{\theta}}$ such that
the functions $\curve_1\left(\alpha_1(\theta)\right) = \bp_1^{\theta}$ and
$\curve_2\left(\alpha_2(\theta)\right) = \bp_2^{\theta}$ are continuous functions from 
$[0, m_1]$ and $[0, m_2]$ to $\reals^{d+1}$, ie. they are continuous traces.
This can be done due to the fact that $R_1$ and $R_2$ are \pprs and thus the
polygons $ R_1\!\left(\alpha_1(\theta)\right)$ and 
$R_2\!\left(\alpha_2(\theta)\right)$ change smoothly with respect to $\theta$.

Observe that the curves $\curve_1$ and $\curve_2$ are such that
\begin{multline*}
\max_{0\leq \theta \leq 1} \norm {\curve_1\!\left(\alpha_1(\theta)\right) - \curve_2\!\left(\alpha_2(\theta)\right)}\\[-1.5mm]
\leq\\[-1mm]
\max_{0\leq \theta \leq 1}\  \Phi_{\min}\Big(
R_1\!\left(\alpha_1(\!\theta\!)\right),\,
R_2\!\left(\alpha_2(\!\theta\!)\right)
\Big)
\end{multline*}
This prove Inequality~\ref{equation:MinInqTheoremProof}.
This concludes the second part of the  theorem proof.
\qedhere
\end{proof}
\end{comment}



==> pipe-distances.tex <==
\section{Distances between Flowpipes}
\label{section:FlowpipeDistances}

\subsection{Basic Definitions}
\label{subsection:Basic}

\noindent\textbf{Traces and Tracepipes.}
A (finite) \emph{trace} or a  \emph{flow}
$f: [T_i,T_e] \rightarrow  \reals^d $ is a  mapping from a
finite closed interval $[T_i,T_e]$ of $\reals_+$,
with $0 \leq T_i < T_e$,
to  $ \reals^d $.
%some topological space  ${\myO}$.
%The time-domain of $f$, denoted $\tdom(f)$, is the time interval $[T_i,T_e]$
over which it is defined.
In this work we restrict our attention to traces which are continuous with respect to time.
A \emph{system} transforms an input trace to an output trace dependent on the initial state of the system.
A \emph{tracepipe} or a \emph{flowpipe} $F$  is a nonempty
collection of traces over some closed interval $[T_i,T_e]$.
%The time-domain of $F$ is denoted $\tdom(F)$.


\smallskip\noindent\textbf{Reachpipes.}
A \emph{reachpipe} $R$ is a mapping  from a
finite closed interval $[T_i,T_e]$  of $\reals_+$, denoted $\tdom(R)$, 
to subsets of $\reals^d$.
The set $R(t)$ denotes the set of reachable values at time $t$.
To a reachpipe $R$, we associate a tracepipe $F^R$ consisting of all continuous traces
$f$  over $\tdom(R) $ such that $f(t) \in R(t)$ for all $t\in \tdom(R)$.
Dually, corresponding to each tracepipe $F$, we associate the reachpipe $R^F$ with the same
domain defined by $R^F(t) =\cup_{f\in F} \set{f(t)}$.
For $C$ the reachpipe corresponding to $F$ (i.e., for  $C=R^F$),
we have $F\subseteq  F^{C}$.
%Note that in general, for a tracepipe $F$, 
Note that in general,
we need not have
$F=  F^{R^F}$, as reachpipes do not carry any flow structure of individual flows;
thus, $ F^{R^F}$ may contain more traces than $F$
(for example, a trace which bounces from one extremity of the pipe to another).

%for $C$ the reachpipe corresponding to $F$ (ie. for  $C=R^F$).
%The tracepipe 

\smallskip\noindent\textbf{Distances between Tracepipes.}
%Let $F_1$ and $F_2$ be two tracepipes.
Consider the setting where tracepipes are generated by systems under initial state 
uncertainty and/or input noise.
Our objective is to quantity the variation in behavior of two systems under this noise and
uncertainty.
With this goal in mind, we define the \emph{variation distance} between
two tracepipes $F_1$ and $F_2$ as follows.
Let $\dist$ be a metric on traces.
%The function $\dist$ is extended to tracepipes as follows:
The variation distance $\dvar(F_1, F_2)$ is defined as
\begin{equation}
\dvar(F_1, F_2) = \sup_{f_1\in F_1, f_2\in F_2} \dist(f_1, f_2)
\end{equation}
%This function $\dist$ over flowpipes is called the variation distance.
We have for all tracepipes $F_1, F_2, F_3$ that
\begin{compactenum}
\item 
$\dvar(F_1, F_2) \geq 0$;
\item $\dvar(F_1, F_2) = \dvar(F_2, F_1)$; and
\item 
$\dvar(F_1, F_3) \leq \dvar(F_1, F_2) + \dvar(F_2, F_3) $.
\end{compactenum}
We may however have $\dvar(F, F) > 0$, thus, $\dvar$ need not be a metric over
tracepipes.
The value $\dvar(F, F) $ gives us the variation amongst traces in $F$ according to 
the original trace metric $\dist$.


%\smallskip\noindent\textbf
\subsection{Estimating Variation Distances 
using Reachpipes}

Tracepipes cannot be constructed for most dynamical systems.
However, reachpipe sets can be over/under-approximated at desired 
timepoints using analytic techniques \cite{ChutinanK03,KurzhanskiV06,Girard05,GirardGM06,GuernicG10,FrehseGDCRLRGDM11,SankaranarayananDI08,ColonS11,ChenAS12}.
Given two tracepipes $F_1, F_2$, and a trace metric $\dist$,
we bound the corresponding tracepipe variation distance $\dvar(F_1, F_2)$ 
using over-approximation reach sets  as follows.

\smallskip\noindent\textbf{Over-approximating the variation distance.}
Let $\ceil{R^{F_1}}$ and $\ceil{R^{F_2}}$ be over-approximations of the reachpipes
$R^{F_1}$ and $R^{F_2}$.
We have 
\begin{equation}
\label{equation:OverApproxReach}
\dvar(F_1, F_2) \leq \dvar\left(F^{\ceil{R^{F_1}}}, F^{\ceil{R^{F_2}}} \right)
\end{equation} 
The above follows from the fact that $F_j \subseteq F^{\ceil{R^{F_j}}}$ for
any tracepipe $F_j$.

\smallskip
\noindent\textbf{Under-approximating the variation distance.}
Consider the Hausdorff distance between the sets $F_1$ and $F_2$, defined by
\begin{equation}
\dist_H(F_1, F_2) = \max\left\{
\sup_{f_1 \in F_1}\inf_{f_2\in F_2}\dist(f_1, f_2)\, , \, \sup_{f_2 \in F_2}\inf_{f_1\in F_1}
\dist(f_1, f_2) \right\}
  \end{equation}
Intuitively, if  $\sup_{f_1 \in F_1}\inf_{f_2\in F_2}\dist(f_1, f_2)$ is less than $\delta$,
then given any trace $f_1\in F_1$, there exists a trace $f_2\in F_2$ such that
$ \dist(f_1, f_2) < \delta$.
Note that $\sup_{f_1 \in F_1}\inf_{f_2\in F_2}\dist(f_1, f_2) \leq \dvar(F_1, F_2)$ and also
 $\sup_{f_2 \in F_2}\inf_{f_1\in F_1}\dist(f_1, f_2) \leq \dvar(F_1, F_2)$, thus, we have
\begin{equation}
\dist_H(F_1, F_2)  \leq \dvar(F_1, F_2)
\end{equation}
%
As mentioned earlier, obtaining tracepipe sets is usually not possible; we have to work with
over or under-approximations.
Unfortunately, there is no obvious relationship between
$\dist_H(A, B) $ and $\dist_H(A', B')$ for $A\subseteq A'$ and $B\subseteq B'$
%$\dist_H\left(F^{\ceil{R^{F_1}}}, F^{\ceil{R^{F_2}}} \right)$.
This can be seen pictorially in Figure~\ref{figure:Hausdorff}.
The set $A, B, A', B'$ are subsets of the interval $[0,10]$.
The the first case  $\dist_H(A, B)  > \dist_H(A', B') $; in the second
 $\dist_H(A, B)  < \dist_H(A', B') $.
\begin{figure}[h]
\strut\centerline{\picfile{hausdorff.eepic}}

\hspace*{-3mm}
\begin{minipage}[t]{0.22\textwidth}
\picfile{hausdorff-2.eepic}
\end{minipage}
$\qquad\ $
\begin{minipage}[t]{0.22\textwidth}
\picfile{hausdorff-3.eepic}
\end{minipage}
\caption{Sets $A, B$, and two cases of $A\subseteq A'$, $B\subseteq B'$}
\label{figure:Hausdorff}
\end{figure}
%
Thus, we cannot use the reachpipe over-approximations  
$\ceil{R^{F_1}}, \ceil{R^{F_2}}$,
 to get a lower bound on
$\dist_H(F_1, F_2)$.
This problem occurs even  even in the case of  exact reachpipes
$R^{F_1}, R^{F_2}$ as $F_1\subseteq  F^{R^{F_1}}$ and 
$F_2\subseteq  F^{R^{F_2}}$.

For the special case where $F_1= \set{f_1}$ is a singleton set, we have
\begin{equation}
\dist_H(\set{f_1}, F_2) = \dvar(\set{f_1}, F_2)
\end{equation}
Thus, in this case of a singleton $F_1$, the value
$\dist_H\left(F^{\ceil{R^{F_1}}}, F^{\ceil{R^{F_2}}} \right)$ only 
gives an upper bound on
$\dvar(F_1, F_2)$.

We note that even if we under-approximate the reach sets to obtain
$F^{\floor{R^{F_1}}}, F^{\floor{R^{F_2}}} $, we still do not have a lower bound for the
Hausdorff distance as we cannot tell in which direction the distance changes on taking
subsets (Figure~\ref{figure:Hausdorff}).
In addition,  we may have $F_j \subset F^{\floor{R^{F_j}}}$ as
$ F^{R^{F_j}}$ over-approximates $F_j$, and competes with the fact that
$\floor{R^{F_j}}$ under-approximates $R^{F_j}$.

Failing to use the Hausdorff distance to get a lower bound, 
we  use the conservative  \emph{minimum set distance}:
\begin{equation}
\dist_{\min}(F_1, F_2) = \inf_{f_1\in F_1, f_2\in F_2} \dist(f_1, f_2)
\end{equation}
For this distance, it is clear that
\[
 \dist_{\min}\left(F^{\ceil{R^{F_1}}}, F^{\ceil{R^{F_2}}} \right) \leq   \dvar(F_1, F_2) 
\]
Combining this with Equation~\ref{equation:OverApproxReach}, we get the following
Proposition.

\begin{proposition}
\label{proposition:OverUnder}
Let $F_1$ and $F_2$ be tracepipes, and let
$\ceil{R^{F_1}}$ and $\ceil{R^{F_2}}$ be over-approximations of the corresponding
reachpipes $R^{F_1}$ and $R^{F_2}$.
We have
\[
\mspace{-15mu}
\dist_{\min}\!\left(\!F^{\ceil{R^{F_1}}}, F^{\ceil{R^{F_2}}} \!\right) \leq   \dvar(F_1, F_2) 
\leq \dvar\!\left(\!F^{\ceil{R^{F_1}}}, F^{\ceil{R^{F_2}}} \!\right).
\mspace{-5mu}\qedhere\qed
\]
\end{proposition}
We note that Proposition~\ref{proposition:OverUnder} holds even if we
take the exact reachpipes, ie., if instead of taking
$\ceil{R^{F_1}}$ and $\ceil{R^{F_2}}$, we take
$R^{F_1}$ and $R^{F_2}$ in the equation of the Proposition.


\smallskip\noindent\textbf{The Pipe Distance Decision Problem in Practice.}
Consider a framework where we want to check if the behaviors of two systems 
over a time interval $[0,T]$
are at most $\delta$ apart, under initial state uncertainty, and 
input signal variation.
The decision schema is presented in Algorithm~\ref{algo:DistancePipe}.
%
\begin{algorithm}[!ht]
\caption{Checking Closeness of Tracepipes}
\label{algo:DistancePipe}
\SetKwInOut{Input}{Input}
  \SetKwInOut{Output}{Output}
  \Input{
    $\system_1, \system_2$  \tcp*{two systems with output values in $\reals^d$}\\
     $X_0^1, X_0^2$   \tcp*{initial state sets of $\system_1, \system_2$}\\
     $U^1, U^2$   \tcp*{class of input signals for $\system_1, \system_2$}\\
     $\dist$ \tcp*{trace metric}\\
     $[0, T]$ \tcp*{time horizon}\\
    $\delta\in \reals_+$  \tcp*{desired tracepipe distance}
}
\Output{Answer to whether $\dvar\left( \system_1\left(X_0^1, U^1\right), \system_2\left(X_0^2, U^2\right)
\right) < \delta$
\tcc*{$\system_j\left(X_0^j, U^j\right)$ is the set of traces of $\system_j$ starting from
$X_0^j$ under inputs from $U^j$}
}
Pick $0=t_0^j < t_1^j < \dots < t_m^j=T$ for $j\in \set{1,2}$\;
\For{$k\in \set{0, 1, \dots, m}$ and $j\in \set{1,2}$}{
Compute over-approximations $\ceil{V_{t_k^j}} \subseteq \reals^d$ of possible trace values at
time ${t_k^j}$ occurring in tracepipe  $\system_j\left(X_0^j, U^j\right)$}
\For{$j\in \set{1,2}$}{
Compute the over-approximate reachpipe $\ceil{R_{\system_j}}$,
 corresponding to tracepipe $\system_j\left(X_0^j, U^j\right)$, from
value sets $\ceil{V_{t_0^j}}, \dots, \ceil{V_{t_m^j}}$
}
$\Delta_L:= \dist_{\min}\left(F^{\ceil{R_{\system_1}}}, F^{\ceil{R_{\system_2}}}\right)$\;
$\Delta_U:= \dvar\left(F^{\ceil{R_{\system_1}}}, F^{\ceil{R_{\system_2}}}\right)$\;
\Switch{$\delta$}{
\uCase{$\delta < \Delta_L$}
{\Return{``System tracepipes $\dvar$ distance exceeds given bound $\delta$}''}
\uCase{$\delta \geq  \Delta_U$}
{\Return{``System tracepipes $\dvar$ distance is under  given bound $\delta$}''}
\uCase{$ \Delta_L \leq  \delta <  \Delta_U$}
{\Return{``System tracepipes $\dvar$ distance range is $[\Delta_L,  \Delta_U)$.
Violation of $\delta$ bound unknown.''}}
}
\end{algorithm}
In case Algorithm~\ref{algo:DistancePipe} returns ``unknown'',  the initial state sets
$X_0, X_1$ or the input signal sets $U_0, U_1$ need to be constrained further
(so as to reduce the width of the reachpipes $\ceil{R_{\system_0}}, \ceil{R_{\system_1}}$),
and the algorithm run again.
The engineer can also compute the Hausdorff distance
$\dist_H\left(F^{\ceil{R_{\system_1}}}, F^{\ceil{R_{\system_2}}}\right)$ to try to get a feel for the 
variation distance $\dvar$.

Special applications of Algorithm~\ref{algo:DistancePipe} are when:
\begin{compactitem}
\item There is no uncertainty in the first  system (eg., when it is a precise 
mathematical model);
this results in the tracepipe of that system having only one trace.
The over-approximation $\ceil{R_{\system_1}}$ of the reachpipe may still end up
having non-zero width due to our inability to precisely compute the reach sets.
\item Both systems (and tracepipes) are the same.
This can arise if we want to check the \emph{robustness}
 of the system under initial state and input perturbations.
\end{compactitem}

In the next section we discuss construction of the reachpipes $\ceil{R_{\system_j}}$
from the value sets $\ceil{V_{t_0^j}}, \dots, \ceil{V_{t_m^j}}$; and also a trace metric
suitable for hybrid systems.
\newpage


==> skoro-pipe.tex <==
\section{Skorokhod Distances between Tracepipes}
\label{section:Skorokhod}

\subsection{The Skorokhod Trace Metric}

The Skorokhod metric allows for  timing as well as trace-value distortions in its
quantification.
Timing distortions are handled using \emph{retiming} functions.
A \emph{retiming} $\retime: I \mapsto  I' $, for closed
intervals $I, I'$ of $\reals_+$   is an order-preserving (i.e., monotone)
continuous
bijective function from
$I$ to $I'$; 
thus if $t<t'$ then $\retime(t) < \retime(t')$.
Let $\retimeclass_{I \mapsto  I' }$
be the class of retiming functions from $I$ to $ I' $
and let $\iden$ be the identity retiming.
Intuitively, retiming can be thought of as follows: imagine a stretchable and compressible
timeline; a retiming  of the original timeline gives a new timeline
 where some parts have been
stretched, and some compressed, without the timeline having been broken.
Given a trace  $f: I_{f} \rightarrow \reals^d$, and a retiming
$\retime: I \mapsto   I_{f} $; the function
$f\circ \retime$ is another trace from $I$ to $\reals^d$.

\begin{definition}[Skorokhod Metric]
Given a retiming $\retime:  I \mapsto I' $, let $||\retime-\iden||_{\sup}$ be defined as
\[
||\retime-\iden||_{\sup} =\sup_{t\in I }|\retime(t)-t|.\]
Given two traces $f: I_{f}\mapsto \reals^d $ and $f': I_{f'} \mapsto \reals^d$,
a metric $\dist_{\reals^d}$ on $\reals^d$,
 and a retiming $\retime:  I_{f} \mapsto   I_{f'}$, let
$\norm{f\,-\, f'\circ \retime}_{\sup}$  be defined as:
\[
\norm{f\,-\, f'\circ \retime}_{\sup}
=
\sup\nolimits_{t\in I_{\pi}} \dist_{\reals^d}\big(\,  f(t)\ ,\ f'\left(\retime(t)\right)\,  \big).\]
The \emph{Skorokhod distance}\footnote{
 The two components
of the Skorokhod distance (the retiming, and the value difference components) can
be weighed with different weights -- this simply corresponds to a change of scale.}
 between the traces  $f()$ and $f'()$  is defined to be:
\begin{equation*}
\label{equation:Skoro}
\dist_{\skoro}(f,f') = \inf_{r\in  \retimeclass_{ I_{f} \mapsto   I_{f'}}}
\max(\norm{\retime-\iden}_{\sup} \, ,\,  \norm{f\,-\, f'\circ \retime}_{\sup}).\qed
\end{equation*}
\end{definition}

Intuitively, the  Skorokhod distance
incorporates two components: the first component quantifies
the {\em timing discrepancy} of the timing distortion required to ``match'' two traces,
and the second quantifies the  \emph{value mismatch}  (in the metric space $\reals^d$)
of the values under the timing distortion.
In the retimed trace $ f\circ \retime$, we see exactly the same values as in $f$, in
exactly the same order, but the times at which the values are seen can be different.
The utility of the  Skorokhod metric has been demonstrated before:
(i)~it provides an appropriate topology for
hybrid systems~ \cite{Broucke98,CaspiB02};
(ii)~close systems under this metric satisfy close logical properties~\cite{DMP15}; and
(iii)~it is tractable to use in a conformance testing framework~\cite{DMP15}.




\subsection{Moving to the \frechet Metric}
\label{subsection:MovingFrechet}

We showed in~\cite{MajumdarP15} that the Skorokhod distance problem between
continuous traces given a point metric $\dist_{\myO}$
can be framed as a \frechet distance problem over related traces and  a related metric.
We employ the same idea to compute distances between reachpipes.


\begin{definition}[\frechet distance]
\label{def:frechet}
Let $\curve_1:[a_1, b_1] \rightarrow {\myV}$ and $\curve_2:[a_2, b_2] \rightarrow {\myV}$ be curves
(a \emph{curve} is a continuous trace where the parameter space need not be interpreted as time).
The \frechet distance between the two curves $f,g$ is defined to be
\[
\dist_{\fre}(\curve_1,\curve_2) = \inf_{\substack{
\alpha_1: [0,1] \rightarrow [a_1, b_1] \\
\alpha_2: [0,1] \rightarrow [a_2, b_2] }}\quad
\max_{0\leq \theta \leq 1} \norm {\curve_1\left(\alpha_1(\theta)\right) - \curve_2\left(\alpha_2(\theta)\right)}
\]
 where $\lVert \, \rVert$ is the norm  over ${\myV}$, and where $\alpha_1, \alpha_2$ range over  continuous and strictly increasing bijective functions
onto $ [a_1, b_1] $ and  $[a_1, b_1] $ respectively.\qed
\end{definition}
Intuitively, the \emph{reparametrizations} $\alpha_1, \alpha_2$ control the ``speed'' of traversal along the
two curves by two entities.
The positions of the two entities in the two curves at ``time'' $\theta$  is given by
$\alpha_1(\theta)$ and $\alpha_2(\theta)$ respectively; with the value of the curves
at those positions being
$ \curve_1\left(\alpha_1(\theta)\right) $ and  $\curve_2\left(\alpha_2(\theta)\right) $ respectively.
The two entities always have a speed strictly greater than $0$.

Let the given point metric on $\reals^d$ be defined in terms of a norm $L$ (eg.,
the $L_1, L_2,$ or $L_{\infty}$ norm).
Given a continuous trace $f: [T_i,T_e] \rightarrow  \reals^d $, we can naturally associate a
curve $\curve_f: [T_i,T_e] \rightarrow  \reals^{d}\times \reals $ where we 
add the time value as an  extra dimension.
Given a value $\tuple{\bp, t} \in \reals^{d}\times \reals$, and a norm $L$ over
$\reals^d$, let the norm $L^{\max}$ be defined by 
\begin{equation}
\label{equation:LMaxDef}
\norm{\tuple{\bp, t}}_{L^{\max}} = \max\left( \norm{\bp}_L, \abs{t}\right).
\end{equation}

\begin{proposition}[From Skorokhod to \frechet~\cite{MajumdarP15}]
\label{proposition:SkoroToFrechet}
Let $f: [T_i^f, T_e^f] \rightarrow \reals^d$ and $g: [T_i^g, T_e^g] \rightarrow \reals^d$ be
two  continuous traces, and let $\reals^d$ have the norm $L$.
We have
\[
\dist_{\skoro}(f,g) =\dist_{\fre}(\curve_f, \curve_g)
 \]
where the curves $\curve_f$ and $ \curve_g$ are the curves in the space
$\reals^d\times \reals$ (with the associated norm
$L^{\max}$)
corresponding to
the traces $f$ and $g$ as defined above. \qed
\end{proposition}


Recall that in Subsection~\ref{subsection:ReachpipeConstruction}, we 
argued for linear interpolation completion of sampled trace values.
The traces so obtained by completion are continuous.
There are hence corresponding curves $C_{f}: [T_i^f, T_e^f]] \rightarrow
\reals^d\times \reals$ for the original traces $f: [T_i^f, T_e^f] \rightarrow
\reals^d$ making Proposition~\ref{proposition:SkoroToFrechet}
applicable.
Corresponding to a tracepipe $F$ over $\reals^d$, there is another related
tracepipe $F^*$ over  $\reals^d\times \reals$ with traces $f\in F$ corresponding
to curves $C_f$ in $F^*$.
We then have
\[
\begin{array}{ll}
{\dist_{\skoro}}_{\var}(F_1, F_2)  & = \sup_{f_1\in F_1, f_2\in F_2} \dist_{\skoro}(f_1, f_2)\\
& =  \sup_{\curve_{f_1}\in F_1^*, \curve_{f_2}\in F_2^*} \dist_{\fre}(\curve_{f_1},\curve_{f_2})\\
& = {\dist_{\fre}}_{\var}(F_1^*, F_2^*) 
\end{array}
\]
We thus henceforth focus on computing the pipe variation distances with respect to 
the \frechet trace metric.





